Monitoring Robustness and Individual Fairness

Input-output robustness appears in various different forms in the literature, such as robustness of AI models to adversarial or semantic perturbations and individual fairness of AI models that make decisions about humans. We propose runtime monitoring of input-output robustness of deployed, black-box AI models, where the goal is to design monitors that would observe one long execution sequence of the model, and would raise an alarm whenever it is detected that two similar inputs from the past led to dissimilar outputs. This way, monitoring will complement existing offline ``robustification'' approaches to increase the trustworthiness of AI decision-makers. We show that the monitoring problem can be cast as the fixed-radius nearest neighbor (FRNN) search problem, which, despite being well-studied, lacks suitable online solutions. We present our tool Clemont, which offers a number of lightweight monitors, some of which use upgraded online variants of existing FRNN algorithms, and one uses a novel algorithm based on binary decision diagrams -- a data-structure commonly used in software and hardware verification. We have also developed an efficient parallelization technique that can substantially cut down the computation time of monitors for which the distance between input-output pairs is measured using the $L_\infty$ norm. Using standard benchmarks from the literature of adversarial and semantic robustness and individual fairness, we perform a comparative study of different monitors in \tool, and demonstrate their effectiveness in correctly detecting robustness violations at runtime.

==> old.tex <==

\newpage
\section{Old}



\smallskip
\noindent\textbf{Adversarial Robustness}
\emph{Setup:} We test our monitor on three standard robustness datasets for the $L_{\infty}$-norm: CIFAR-10 and CIFAR-100 each restricted to $10000$ $32\times32$ color images \cite{krizhevsky2009learning}; ImageNet restricted to $5000$ \cite{deng2009imagenet} $256\times 256$ color images. We enrich each dataset, by adding a adversarial example for each entry using the RobustBench's \cite{croce2020robustbench} included adversarial attack feature.
For each dataset we train classifiers using the worst and best performing method from RobustBench, i.e. we select respectively the trainings procedure from: 
Croce et.al.~\cite{croce2020robustbench} and Bartoldson et.al.~\cite{bartoldson2024adversarial} for CIFAR-10; Rice et.al.~\cite{rice2020overfitting} and Wang et.al.~\cite{wang2023better} for CIFAR-100; Croce et.al.~\cite{croce2020robustbench} and Amini et.al.~\cite{amini2024meansparse} for ImageNet. The distance is measured using $L_{\infty}$ with $\epsilon$ set to $\frac{8}{255}$ for CIFAR-$\{10,100\}$ and $\frac{4}{255}$ for ImageNet.
\emph{Results:} The monitor identifies $100\%$ of all adversarial attacks. Moreover, the number of successful adversarial attacks detected by our monitor is in accordance to the RobustBench's leaderboard (see Table~\ref{tab:adversarial_results}).

% \begin{table}[h]
% \centering
% \begin{tabular}{lccccc}
% \hline
% Dataset & Model & $\epsilon$ & \#Adversarials & \#Positives \\
% \hline
% \multirow{2}{*}{CIFAR-10} & Bartoldson* & \multirow{2}{*}{$\frac{8}{255}$} & 1,962 & 1,962 \\
% & Standard & & 9,477 & 9,477 \\
% \hline
% \multirow{2}{*}{CIFAR-100} & Wang* & \multirow{2}{*}{$\frac{8}{255}$} & 3,156 & 3,156 \\
% & Rice & & 3,438 & 3,438 \\
% \hline
% \multirow{2}{*}{ImageNet} & Amini* & \multirow{2}{*}{$\frac{4}{255}$} & 930 & 930  \\
% & Standard & & 3,836 & 3,836 \\
% \hline
% \end{tabular}
% \caption{Monitoring outcome for adversarial robustness benchmarks: Model performance across different datasets. Procedure: 1) Take 10k images for CIFAR models, 5k images for ImageNet models. 2) Run the adversarial attacker provided by RobustBench on the images. This produces another 10k or 5k images, some of which will have been successfully perturbed to fool the model (\#Adversarials). 3) Run the monitor on combined 20k or 10k sequence of images and decisions, and count the flags (\#Positives)}
% \label{tab:adversarial_results}
% \end{table}



 \smallskip \noindent\textbf{Semantic Robustness}

\emph{Setup:} We test our monitor on three standard robustness datasets for common corruptions: CIFAR-10-C and CIFAR-100-C each restricted to $10000$ $32\times32$ color images \cite{krizhevsky2009learning}; ImageNet-3DCC restricted to $5000$ \cite{deng2009imagenet} $256\times 256$ color images. We enrich each dataset, by adding a adversarial example for each entry using the RobustBench's \cite{croce2020robustbench} included common corruption feature.
We do this exhaustively for all available corrupted versions, meaning all combinations of severity and type of corruption.
To measure the semantic closeness of two images, we use Meta's DINOv2 embedding model, which is designed for the robustness use case \cite{oquab2023dinov2}. 
For each dataset we train classifiers using the worst and best performing method from RobustBench, i.e. we select respectively the trainings procedure from: 
Croce et.al.~\cite{croce2020robustbench} and Diffenderfer et.al.~\cite{diffenderfer2021winning} for CIFAR-10-C; Erichson et.al.~\cite{erichson2022noisymix} and Gowal et.al.~\cite{gowal2020uncovering} for CIFAR-100-C; Krizhevsky et.al.~\cite{krizhevsky2012imagenet} and Tian et.al.~\cite{tian2022deeper} for ImageNet-3DCC.
The input to the monitor is a stream consisting of the embedding given by DINOv2 and the prediction of the model for each image in the data set. The distance is measured using the $L_2$-norm with $\epsilon$ set to $7.5$ for CIFAR-$\{10,100\}$-C and $12.5$ for ImageNet-3DCC. 
\emph{Results:} The monitor detects less violations for robust models. Counterintuitively, as the corruption severity increases, the number of detected violations decreases, with the contrast corruption being an exception. We suspect that in most cases an increase in severity results in a large difference in the embedding space, thus leading to a small number of violations. The opposite dynamic can be observed for contrast corruption.


\begin{figure}
    \centering
    \begin{tabular}{cc}
        \includegraphics[width=0.45\linewidth]{figures/cifars.png} & 
        \includegraphics[width=0.45\linewidth]{figures/imagenet.png} 
    \end{tabular}
    \caption{Percentage of True Positives identified by monitor in semantic usecase across datasets. Left: CIFAR datasets, Right: ImageNet.}
    \label{fig:combined-heatmap}
\end{figure}



% \begin{figure}
%     \centering
%     \includegraphics[width=1\linewidth]{figures/cifars.png}
%     \caption{Percentage of True Positives identified by monitor in semantic usecase on CIFAR datasets. Left to right: Top CIFAR-100C model, Bottom CIFAR-100C model, Top CIFAR-10C model, Bottom CIFAR-10C model. Ranked by Adversarial Accuracy on RobustBench leaderboard.}
%     \label{fig:cifars-heatmap}
% \end{figure}
% \begin{figure}
%     \centering
%     \includegraphics[width=1\linewidth]{figures/imagenet.png}
%     \caption{Percentage of True Positives identified by monitor in semantic usecase on ImageNet. Left to right: Top ImageNet-3DCC model, Bottom ImageNet-3DCC model. Ranked by Adversarial Accuracy on RobustBench leaderboard.}
%     \label{fig:imagenet-heatmap}
% \end{figure}




 \smallskip \noindent\textbf{Individual Fairness}
\emph{Setup:} We test our monitor on three standard fairness datasets: the German Credit dataset consisting of $1000$ entries with $20$ features \cite{german}; 
the Adult Census Income dataset consisting of $48842$ entries with $14$ features \cite{adult}; 
the COMPAS dataset consisting of $6172$ entries with $14$ features \cite{?}.
For each dataset we train a baseline and a fair classifier using the procedure: LCIFR by Ruoss et.al.~\cite{ruoss2020learning}; CertiFair by Khedr et.al.~\cite{khedr2023certifair}. 
\emph{Results:} The monitor detects a greater number of fairness violations for baseline models than fair models. The number of flags raised for models trained according to CertiFair are greater than for LCIFR (see Table~\ref{tab:air_results}). 
\todo{ask david about "fair" model being unfair? And about local vs global}





\KM{David's write-up:}
All experiments follow the same basic structure. We obtain a sequence of input vectors and model predictions and run the monitor on this data. 

The pipeline saves a .json file with the results from the run. This includes metadata, any identified counterexamples and timing information.

There are pre-made scripts to easily reproduce every experiment.

\subsection{Adversarial robustness usecase}

Input data: RobustBench. There are several leaderboards for adversarial attacks under Linf norm, see \url{https://robustbench.github.io/#leaderboard}. We use CIFAR-10 Linf, CIFAR-100 Linf, and ImageNet Linf leaderboards. From these we pick the best and worst performing models. Then we take a subset of the dataset (n=10,000 in case of CIFAR, n=5,000 in case of ImageNet) and use RobustBench's included adversarial attack feature (detailed here \url{https://robustbench.github.io/#leaderboard}) to generate adversarial examples from the original images. We concatenate the original images and adversarial examples into one unified sequence, and obtain model predictions for the full sequence. Then the monitor runs on the whole sequence. If there is a successful adversarial attack, then the sequence contains the original image, with the original (correct) model prediction, as well as the adversarial example, which is epsilon-close to the original, but has a different, incorrect model prediction. The monitor should be able to identify these successful adversarial attacks.

What do we look at: Monitor counterexamples with Linf eps=8/255 for CIFAR, 4/255 for ImageNet.

Questions: Does it find all the attacks? Do robust models indeed perform better?

\begin{table}[h]
\centering
\begin{tabular}{lccccc}
\hline
Dataset & Model & $\epsilon$ & \#Adversarials & \#Positives \\
\hline
\multirow{2}{*}{CIFAR-10} & Bartoldson* & \multirow{2}{*}{$\frac{8}{255}$} & 1,962 & 1,962 \\
& Standard & & 9,477 & 9,477 \\
\hline
\multirow{2}{*}{CIFAR-100} & Wang* & \multirow{2}{*}{$\frac{8}{255}$} & 3,156 & 3,156 \\
& Rice & & 3,438 & 3,438 \\
\hline
\multirow{2}{*}{ImageNet} & Amini* & \multirow{2}{*}{$\frac{4}{255}$} & 930 & 930  \\
& Standard & & 3,836 & 3,836 \\
\hline
\end{tabular}
\caption{Monitoring outcome for adversarial robustness benchmarks: Model performance across different datasets. Procedure: 1) Take 10k images for CIFAR models, 5k images for ImageNet models. 2) Run the adversarial attacker provided by RobustBench on the images. This produces another 10k or 5k images, some of which will have been successfully perturbed to fool the model (\#Adversarials). 3) Run the monitor on combined 20k or 10k sequence of images and decisions, and count the flags (\#Positives)}
\label{table:model_performance}
\end{table}


Takeaways: Yes to both. The monitor indeed identifies 100\% of successful adversarial attacks in all experiments. We can also see that robust models have fewer inputs flagged, because there are fewer successful adversarial attacks (our numbers are in accordance with the ones listed in RobustBench's leaderboard), though sometimes the attacks still succeed, and monitoring identifies this.

Still todo: We could show some of the concrete adversarial images fooling even robust models. But I think this is not particularly novel/interesting.

\subsection{Semantic robustness usecase}

Input data: RobustBench Corruptions leaderboards, see again \url{https://robustbench.github.io/#leaderboard}. This time we use CIFAR-10C, CIFAR-100C, and ImageNet-3dcc. Pick again the best and worst performing models. Again we take a subset of the original dataset (n=10,000 in case of CIFAR, n=5,000 in case of ImageNet) and the same subset of a corrupted version of the dataset. We do this exhaustively for all available corrupted versions, meaning all combinations of severity and type of corruption. Again concatenate the original and corrupted images into one sequence. For this sequence, we obtain the classifier predictions, as well as the embedding vectors for each image according to Meta's DINOv2 embedding model, see \url{https://github.com/facebookresearch/dinov2}. This embedding model is specifically targeted at robustness. The monitor's input sequence then consists of these embeddings, paired with the classifier predictions for the corresponding original image. If the model flips its prediction for a corrupted image, but the embedding model gives an epsilon-close embedding for the corrupted image, then the monitor is going to throw a flag. Note this could technically work with other embeddings, like text, without changes to the monitor.

What do we look at: Monitor counterexamples with L2 eps=7.5 for CIFAR, 12.5 for ImageNet. (Use L2 over Linf because Linf doesn't play well with embeddings. L2 is common)

Questions: 

\begin{enumerate}
    \item Does this embedding idea work?
    \item What are the trends across corruption/severity pairings and models?
    \item Are there interesting counterexamples?
\end{enumerate}
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/cifar10c-Diffenderfer2021Winning_LRR_CARD_Deck_heatmap.png}
    \caption{Performance of the top adversarial accuracy model (Diffenderfer) on the CIFAR-10-C dataset.}
    \label{fig:cifar10c-diffenderfer-top}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/cifar10c-Standard_heatmap.png}
    \caption{Performance of the baseline model ("Standard") on the CIFAR-10-C dataset.}
    \label{fig:cifar10c-standard-bottom}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/cifar100c-Diffenderfer2021Winning_LRR_CARD_Deck_heatmap.png}
    \caption{Performance of the top adversarial accuracy model (Diffenderfer) on the CIFAR-100-C dataset.}
    \label{fig:cifar100c-diffenderfer-top}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/cifar100c-Gowal2020Uncovering_Linf_heatmap.png}
    \caption{Performance of the bottom adversarial accuracy model (Gowal) on the CIFAR-100-C dataset.}
    \label{fig:cifar100c-gowal}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/imagenet3dcc-Tian2022Deeper_DeiT-B_heatmap.png}
    \caption{Performance of the top adversarial accuracy model (Tian) on the ImageNet-3D-CC dataset.}
    \label{fig:imagenet3dcc-tian}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/imagenet3dcc-AlexNet_heatmap.png}
    \caption{Performance of the baseline model (AlexNet) on the ImageNet-3D-CC dataset.}
    \label{fig:imagenet3dcc-alexnet}
\end{figure}

Takeaways: ad 1,2) This is best seen from the heatmaps. Robust models indeed see less inputs flagged across the board. Then there are large differences depending on which corruption is used. Also, you might expect that as the severity increases, there are more inputs flagged. This is not actually so in many cases, and I suspect it is because the embedding model starts mapping severely corrupted inputs to distant embedding vectors, so the monitor doesn't care if the model decision flips as well. Finally there's an outlier with the contrast corruption, which I believe is the opposite thing happening: the embedding model tends to map inputs with this particular corruption to close embedding vectors, because these images almost look like a flat color, resulting in a lot of flags raised.

Noet also this is straightforward to retrofit to any vision model, and acts like an almost free extra layer of security, a second pair of eyes so to say.

Still todo: 3) It might be interesting to show concrete corrupted images that fool the classifier, in particular to support the idea that one can get human review in the loop.

\subsection{Fairness usecase}

Input data:

\begin{itemize}
    \item German Credit dataset - A credit risk dataset of 1000 loan applications, classifying applicants as good or bad credit risks based on 20 features including age, employment, credit history. From UCI ML: \url{https://archive.ics.uci.edu/ml/datasets/statlog+(german+credit+data)}
    \item Adult Census Income dataset - Also known as "Census Income" dataset, contains ~48,000 instances predicting whether income exceeds \$50K/yr based on census data (age, education, occupation etc). From UCI ML: \url{https://archive.ics.uci.edu/ml/datasets/adult}
    \item COMPAS dataset - ProPublica's analysis of COMPAS recidivism algorithm data, containing ~7,000 criminal defendant records used to assess likelihood of recidivism. Used to study algorithmic bias in criminal justice. Available at: \url{https://github.com/propublica/compas-analysis}
\end{itemize}

We obtain predictions for these datasets from two other works: lcifr \url{https://github.com/eth-sri/lcifr}, and CertiFair \url{https://github.com/rcpsl/Certifair} These works propose methodologies to train fair models. Both provide code to train baseline and fair models on these 3 datasets. For lcifr, there are several fairness constraints, we train the fair model according to the "Noise" constraint because this corresponds directly to epsilon-fairness. For CertiFair, relevant for us is what they call "P2" property (see the "Fairness properties" paragraph, p.6) 

What do we look at:  Monitor counterexamples with Linf eps TBD

Questions: Do fair models perform better? How do concrete "unfair" decisions look like? 
% \begin{table}
% \small
% \centering
% \begin{tabular}{|c|c|c|c|c|c|c|}
% \hline
% \textbf{Dataset} & \textbf{$\epsilon$} & \textbf{LBase} & \textbf{LFair} & \textbf{CBase} & \textbf{CLocal} & \textbf{CGlobal} \\
% \hline
% \multirow{12}{*}{Adult} 
% & 0.0025 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
% & 0.005 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
% & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
% & 0.02 & 0.00 & 0.00 & 0.15 & 0.18 & 0.00 \\
% & 0.04 & 0.00 & 0.00 & 3.35 & 1.74 & 0.04 \\
% & 0.08 & 0.01 & 0.00 & 14.61 & 14.40 & 0.55 \\
% & 0.12 & 0.01 & 0.00 & 19.23 & 20.71 & 1.40 \\
% & 0.16 & 0.06 & 0.00 & 23.15 & 26.31 & 2.49 \\
% & 0.20 & 0.07 & 0.00 & 24.81 & 28.54 & 2.96 \\
% & 0.24 & 0.15 & 0.01 & 27.23 & 32.18 & 4.04 \\
% & 0.28 & 0.19 & 0.01 & 28.66 & 34.39 & 4.55 \\
% & 0.32 & 0.36 & 0.03 & 30.15 & 36.35 & 5.03 \\
% \hline
% \multirow{12}{*}{COMPAS}
% & 0.0025 & 0.00 & 0.00 & 0.09 & 0.00 & 0.08 \\
% & 0.005 & 0.00 & 0.00 & 0.30 & 0.02 & 0.17 \\
% & 0.01 & 0.00 & 0.00 & 0.34 & 0.13 & 0.30 \\
% & 0.02 & 0.02 & 0.00 & 1.36 & 0.81 & 1.04 \\
% & 0.04 & 0.14 & 0.00 & 11.90 & 8.49 & 7.90 \\
% & 0.08 & 0.33 & 0.00 & 30.25 & 33.91 & 22.64 \\
% & 0.12 & 1.68 & 0.19 & 40.97 & 49.08 & 33.11 \\
% & 0.16 & 1.80 & 0.19 & 55.37 & 59.73 & 40.59 \\
% & 0.20 & 3.91 & 0.47 & 60.07 & 63.71 & 42.38 \\
% & 0.24 & 11.03 & 3.62 & 66.81 & 70.94 & 47.00 \\
% & 0.28 & 13.47 & 4.14 & 68.97 & 72.85 & 48.06 \\
% & 0.32 & 13.85 & 4.26 & 72.65 & 74.31 & 48.76 \\
% \hline
% \multirow{12}{*}{German}
% & 0.0025 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
% & 0.005 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
% & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
% & 0.02 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
% & 0.04 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
% & 0.08 & 0.00 & 0.00 & 0.60 & 0.60 & 0.00 \\
% & 0.12 & 0.00 & 0.00 & 1.70 & 3.00 & 0.00 \\
% & 0.16 & 0.00 & 0.00 & 2.90 & 4.40 & 0.00 \\
% & 0.20 & 0.00 & 0.00 & 3.30 & 5.09 & 0.00 \\
% & 0.24 & 0.00 & 0.00 & 6.59 & 8.19 & 0.00 \\
% & 0.28 & 0.00 & 0.00 & 12.89 & 13.89 & 0.50 \\
% & 0.32 & 0.00 & 0.00 & 15.18 & 15.68 & 0.60 \\
% \hline
% \end{tabular}
% \caption{Percentage of flagged inputs for different datasets, $\epsilon$ values, and methods. LBase - Lcifr baseline model, LFair - Lcifr fair model, CBase - Certifair baseline model, CLocal - Certifair locally regularized (?), CGlobal - Certifair globally regularized (?).}
% \label{tab:results}
% \end{table}

\iffalse
Old table using absolute numbers of counterexample pairs found.
\begin{table}
\small
\centering
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\textbf{Dataset} & \textbf{$\epsilon$} & \textbf{LBase} & \textbf{LFair} & \textbf{CBase} & \textbf{CLocal} & \textbf{CGlobal} \\
\hline
\multirow{12}{*}{Adult} 
& 0.0025 & 0 & 0 & 0 & 0 & 0 \\
& 0.005 & 0 & 0 & 0 & 0 & 0 \\
& 0.01 & 0 & 0 & 1 & 1 & 0 \\
& 0.02 & 0 & 0 & 105 & 120 & 0 \\
& 0.04 & 0 & 0 & 3,570 & 1,588 & 37 \\
& 0.08 & 2 & 0 & 45,890 & 39,732 & 557 \\
& 0.12 & 3 & 0 & 83,799 & 76,448 & 1,725 \\
& 0.16 & 20 & 0 & 130,118 & 120,363 & 4,321 \\
& 0.20 & 26 & 0 & 154,906 & 143,562 & 5,785 \\
& 0.24 & 57 & 2 & 191,368 & 178,609 & 9,652 \\
& 0.28 & 82 & 4 & 216,199 & 201,746 & 11,778 \\
& 0.32 & 161 & 8 & 233,817 & 217,556 & 14,006 \\
\hline
\multirow{12}{*}{COMPAS} 
& 0.0025 & 0 & 0 & 8 & 0 & 6 \\
& 0.005 & 0 & 0 & 20 & 1 & 13 \\
& 0.01 & 0 & 0 & 22 & 7 & 26 \\
& 0.02 & 1 & 0 & 168 & 54 & 117 \\
& 0.04 & 10 & 0 & 5,076 & 1,148 & 1,233 \\
& 0.08 & 24 & 0 & 15,648 & 10,226 & 6,002 \\
& 0.12 & 265 & 9 & 24,717 & 19,676 & 11,266 \\
& 0.16 & 280 & 9 & 46,207 & 35,969 & 17,526 \\
& 0.20 & 773 & 31 & 57,074 & 45,509 & 21,511 \\
& 0.24 & 2,679 & 369 & 70,312 & 58,045 & 25,922 \\
& 0.28 & 3,754 & 526 & 77,139 & 65,629 & 29,824 \\
& 0.32 & 3,922 & 547 & 83,565 & 72,735 & 32,066 \\
\hline
\multirow{12}{*}{German} 
& 0.0025 & 0 & 0 & 0 & 0 & 0 \\
& 0.005 & 0 & 0 & 0 & 0 & 0 \\
& 0.01 & 0 & 0 & 0 & 0 & 0 \\
& 0.02 & 0 & 0 & 0 & 0 & 0 \\
& 0.04 & 0 & 0 & 0 & 0 & 0 \\
& 0.08 & 0 & 0 & 6 & 6 & 0 \\
& 0.12 & 0 & 0 & 22 & 45 & 0 \\
& 0.16 & 0 & 0 & 54 & 87 & 0 \\
& 0.20 & 0 & 0 & 66 & 103 & 0 \\
& 0.24 & 0 & 0 & 157 & 206 & 0 \\
& 0.28 & 0 & 0 & 398 & 524 & 5 \\
& 0.32 & 0 & 0 & 505 & 653 & 8 \\
\hline
\end{tabular}
\caption{Number of true positives for different datasets, $\epsilon$ values, and methods. LBase - Lcifr baseline model. LFair - Lcifr fair model. CBase - Certifair baseline model. CLocal - Certifair locally fair regularizer (??). CGlobal - Certifair globally fair regularizer.}
\label{table:true_positives_extended}
\end{table}
\fi




Takeaways: Fair models indeed perform much better. But there remain some instances of "unfair" decisions. In the appendix there are concrete inputs producing unfair decisionmaking for both a standard and a fair model. There are 4 unfair pairs for the fair model, and 28 for the standard model.

Furthermore, a "fair" model trained for some fairness objective may produce less fair decisions when considering another fairness objective. In the experiment in the appendix, the monitor was blinded to the "race" column (meaning a difference in the "race" column was not taken to mean that two samples are distant, while this did hold for the rest of the categorical columns). All of the four unfair decisions produced by the the fair model have no meaningful differences besides the "race" column. So it would indeed be 100\% fair on the tested sample, if not for the monitor being blinded to race. The standard model produces far more unfair pairs, but only two pairs have race differences. So the fair model actually makes twice as many unfair decisions w.r.t race. (It's well established that different fairness objectives are inherently at odds, but being able to monitor for this is certainly an advantage. You can also imagine running multiple monitors, each on a different fairness objective, to see how the balance is)

Still todo: We don't have numbers for all the models yet, only the concrete counterexamples in the appendix. Produce a table with the number of flagged inputs for baseline, lcifr, CertiFair models, in each of the three datasets. Need to settle on epsilon, too.

\subsection{Comparison of backends}

\subsubsection{Scaling in the number of processed samples}

Input: HIGGS dataset, 10.5m rows \url{https://archive.ics.uci.edu/dataset/280/higgs}. I am running this experiment twice, once on full 22 dimensions of HIGGS, once on 12 (BDD should perform much better there)

What do we look at: Time to process a sample

Questions: How does this develop as the runtime progresses?
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/performance/11-0.01.png}
    \caption{10m rows in 12d (first 12 columns from HIGGS dataset) eps=0.01. Line shows rolling average with 100k window size. Batch size is 10k for batched methods kdtree, SNN. Timeout at 36h. Legend: Blue - BDD, Orange - Brute force, Green - Kdtree Linf, Red - Kdtree L2, Purple - SNN, Brown dashed - BDD @2threads, Pink dashed - Kdtree @2threads}
    \label{fig:12d-0.01}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/performance/11-0.025.png}
    \caption{10m rows in 12d (first 12 columns from HIGGS dataset) eps=0.025. Line shows rolling average with 100k window size. Batch size is 10k for batched methods kdtree, SNN. Timeout at 36h}
    \label{fig:12d-0.025}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/performance/11-0.05.png}
    \caption{10m rows in 12d (first 12 columns from HIGGS dataset) eps=0.05. Line shows rolling average with 100k window size. Batch size is 10k for batched methods kdtree, SNN. Timeout at 36h}
    \label{fig:12d-0.05}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/performance/23-0.01.png}
    \caption{10m rows in 24d (first 24 columns from HIGGS dataset) eps=0.01. Line shows rolling average with 100k window size. Batch size is 10k for batched methods kdtree, SNN. Timeout at 36h}
    \label{fig:24d-0.01}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/performance/23-0.025.png}
    \caption{10m rows in 24d (first 24 columns from HIGGS dataset) eps=0.025. Line shows rolling average with 100k window size. Batch size is 10k for batched methods kdtree, SNN. Timeout at 36h}
    \label{fig:24d-0.025}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/performance/23-0.05.png}
    \caption{10m rows in 24d (first 24 columns from HIGGS dataset) eps=0.05. Line shows rolling average with 100k window size. Batch size is 10k for batched methods kdtree, SNN. Timeout at 36h}
    \label{fig:24d-0.05}
\end{figure}



Takeaways: None yet

Still todo: Wait for completion and plot the throughput

\subsubsection{Scaling in the number of dimensions}

Input: Imagenet data (150k dimensions) where we progressively cut dimensions (e.g. try with 10d, 20d, 40d, ...)

What do we look at: Average time to process a sample.

Questions: How does this develop as the dimensions go up?

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/performance/dimensions.png}
    \caption{Runtime in dimensions. This was done by taking 10k images from ImageNet, which are 224x224px, 3 color channels, giving 150528 dimensions total. For each experiment, I dropped increasingly larger subsets of the dimensions before feeding the input sequence to the monitor. In this experiment, Gaussian noise was added to the 10,000 samples to obtain 100k random samples to feed to the monitor. The plot shows the average processing time for processing another 10k samples, after preloading 100k. (the subsets to drop were determined randomly but with a fixed seed. The predictions were reassigned into 10 classes, down from ImageNet's original 1000 classes.)}
    \label{fig:dimensions}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/parallelization.png}
    \caption{Runtime in dimensions for the parallel methods. This uses the same data as the dimension comparison but without preloading 100k samples due to worker synchronization issues with the preloading.}
    \label{fig:parallelization}
\end{figure}

Still todo: Set this experiment up, run it, and plot it.






\section{Survey}
Surveys
\begin{itemize}
    \item \cite{bhatia2010survey}: \href{https://staff.fmi.uvt.ro/~daniela.zaharie/dm2018/EN/Projects/Biblio/kNN/NearestNeighborSurvey.pdf}{(L1)}
\end{itemize}
\subsection{Dynamic}
\begin{itemize}
    \item ?? \cite{naidan2012static}: \href{https://folk.idi.ntnu.no/mlh/hetland_org/research/2012/static.pdf}{(L1)}
     \item Dynamic VP-Tree \cite{fu2000dynamic}: \href{https://link.springer.com/content/pdf/10.1007/PL00010672.pdf}{(L1)}
     \item DSACL Tree: \cite{britos2012dsacl}: \href{https://www.academia.edu/download/80806759/978-3-642-32153-5_9.pdf}{(L1)}
\end{itemize}

\subsection{Fixed-Radius Neighbour Search}
Fixed-Radius Neighbour Search (RNN) aims at identifying all data points within a given distance from a query point

The most recent work on RNN is by Chen et.al.~\cite{chen2024fast}. Their algorithm sorts the data points by their first principal component to prune the query search space. In their implementation they use Basic Linear Algebra Subprograms (BLAS) to gain additional efficiency.



\subsection{K-Nearest Neighbour Search}
K Nearest Neighbour Search aims at identifying the k-nearest points from a query point.




\subsection{Survey Approximate}
To speedup NN search, modern approaches generally focus on two aspects, namely indexing and sketching. The indexing aims to construct a data structure that prunes the search space for a given query, hopefully resulting in fewer distance computations. Sketching, on the other hand, aims at reducing the cost of each distance computation by using a compressed approximate representation of the data.

\begin{itemize}
    \item K-D Tree \cite{bentley1975multidimensional,friedman1977algorithm}: \href{https://dl.acm.org/doi/pdf/10.1145/361002.361007}{(L1)} \href{https://dl.acm.org/doi/pdf/10.1145/355744.355745}{(L2)};
    \item Ball Tree \cite{omohundro1989five}: \href{https://citeseerx.ist.psu.edu/document?repid=rep1&type=pdf&doi=28fd6c26d45eec7b7586e28e3a5cfef2a7b1375c}{L1}
    \item VP-Tree \cite{yianilos1993data}: \href{https://www.academia.edu/download/72297886/Data_structures_and_algorithms_for_neare20211012-8944-15jug6a.pdf}{L1}
   
    \item Cover Tree \cite{beygelzimer2006cover}: \href{https://dl.acm.org/doi/pdf/10.1145/1143844.1143857}{(L1)}
    \item RP Tree \cite{dasgupta2013randomized}: \href{http://proceedings.mlr.press/v30/Dasgupta13.pdf}{(L1)}
    \item FLANN (Priority Search K-Means Tree ) \cite{muja2009flann,muja2014scalable}:  \href{https://www.cs.ubc.ca/research/flann/uploads/FLANN/flann_manual-1.8.4.pdf}{(L1)}, \href{https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=6809191}{(L2)}
    \item Random KD tree \cite{ram2019revisiting}: \href{https://dl.acm.org/doi/pdf/10.1145/3292500.3330875}{(L1)}
    \item GriSPy \cite{chalela2021grispy}: \href{https://www.sciencedirect.com/science/article/am/pii/S2213133720300974}{(L1)}
    \item 
\end{itemize}




\subsection{K-Nearest Neighbour Search}
Algorithms for KNN:
\begin{itemize}
    \item Randomized k-d trees \cite{silpa2008optimised}:  \href{https://citeseerx.ist.psu.edu/document?repid=rep1&type=pdf&doi=834b4a31f33ccdbf4a92aa004031318df015f825}{(L1)} 
    \item  Hierarchical k-means \cite{nister2006scalable}: \href{https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=1641018}{(link)}
    \item Local Sensitivity Hashing \cite{indyk1998approximate}: \href{https://dl.acm.org/doi/pdf/10.1145/276698.276876}{(link)}.
    \item HNSW \cite{malkov2018efficient,malkov2012scalable}: \href{https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=8594636}{(L1)} , \href{https://www.researchgate.net/profile/Alexander-Ponomarenko/publication/262334462_Scalable_Distributed_Algorithm_for_Approximate_Nearest_Neighbor_Search_Problem_in_High_Dimensional_General_Metric_Spaces/links/5412d49b0cf2bb7347db0da8/Scalable-Distributed-Algorithm-for-Approximate-Nearest-Neighbor-Search-Problem-in-High-Dimensional-General-Metric-Spaces.pdf}{L2}
    \item ScaNN \cite{guo2020accelerating}:   \href{http://proceedings.mlr.press/v119/guo20h/guo20h.pdf}{(link)}
    \item Neural Local Sensitivity Hashing \cite{dong2019learning}: \href{https://arxiv.org/pdf/1901.08544}{(L1)}
\end{itemize}



\subsection{Implementations}

\begin{itemize}
    \item \href{https://github.com/google-research/google-research/tree/master/scann}{ScaNN}
    \item \href{https://pynndescent.readthedocs.io/}{PyNNDescent} 
    \item \href{https://github.com/nmslib/hnswlib}{hnswlib}
    \item \href{https://github.com/nmslib/nmslib}{nmslib} (sort of a superset of hnswlib, but critically, no incremental indexing in its hnsw implementation)
\end{itemize}

\subsection{Notions of fairness}

\begin{itemize}
    \item \href{https://dl.acm.org/doi/pdf/10.1145/3631326}{Bias Mitigation for Machine Learning Classifiers: A Comprehensive Survey} June 2024, section 6 lists fairness metrics
    \item \href{https://arxiv.org/pdf/2002.10312}{Learning Certified Individually Fair Representations} 2020, appendix H
    \item \href{https://dl.acm.org/doi/abs/10.1145/3494672}{A Review on Fairness in Machine Learning} 2022, section 3
\end{itemize}

\subsection{IDK}

\begin{itemize}
    \item Similarity search: the metric space approach \cite{zezula2006similarity}: \href{https://web.iitd.ac.in/~sumeet/Similarity%20Search.pdf}{(L1)}
\end{itemize}

==> survey.tex <==

\section{Survey}



\subsection{Nearest Neighbours}


\subsubsection{Tree Based Methods}
They are all instances of metric trees. A metric tree is any tree data structure specialized to index data in metric spaces. Metric trees exploit properties of metric spaces such as the triangle inequality to make accesses to the data more efficient. 
Of particular interest are R-trees as they are designed for a dynamical setting. 





\paragraph{R-Tree and $R^*$ Trees}
The key idea of the data structure is to group nearby objects and represent them with their minimum bounding rectangle in the next higher level of the tree. Since all objects lie within this bounding rectangle, a query that does not intersect the 
bounding rectangle also cannot intersect any of the contained objects. At the leaf level, each rectangle describes a single object; at higher levels the aggregation includes an increasing number of objects. This can also be seen as an increasingly coarse approximation of the data set. 
This data structure has a bad-worst case complexity, but may perform well in practice. If the bounding boxes do not overlap, search is $O(\log n)$ and insertion is $O(\log n)$. Otherwise both can be $O(n)$.
$R^*$-trees trade a slightly higher construction cost for an increased query speed.

\paragraph{Ball Trees}
A ball tree is a binary tree in which every node defines a D-dimensional ball containing a subset of the points to be searched. Each internal node of the tree partitions the data points into two disjoint sets which are associated with different balls. While the balls themselves may intersect, each point is assigned to one or the other ball in the partition according to its distance from the ball's center. Each leaf node in the tree defines a ball and enumerates all data points inside that ball.
Both search and insertion are $O(\log n)$.

\paragraph{VP-tree}
A vantage-point tree (or VP tree) is a metric tree that segregates data in a metric space by choosing a position in the space (the "vantage point") and partitioning the data points into two parts: those points that are nearer to the vantage point than a threshold, and those points that are not. By recursively applying this procedure to partition the data into smaller and smaller sets, a tree data structure is created where neighbours in the tree are likely to be neighbours in the space.
It requires $O(n)$ memory, it requires $O(k\log n)$ time to add an element, a nearest neighbour query can be performed in $O(k \log n)$ where $k$ is the number of vantage points

\paragraph{Cover Tree}
The tree can be thought of as a hierarchy of levels with the top level containing the root point and the bottom level containing every point in the metric space. Each level $C$ is associated with an integer value $i$ that decrements by one as the tree is descended. 
It requires $O(n)$ memory, it requires $O(c^6\log n)$ time to add an element, a nearest neighbour query can be performed in $O(c^{12} \log n)$ where $c$ is the expansion constant of the data set. 


\paragraph{K-D Tree}
The k-d tree is a binary tree in which every node is a k-dimensional point. Every non-leaf node can be thought of as implicitly generating a splitting hyperplane that divides the space into two parts, known as half-spaces. Points to the left of this hyperplane are represented by the left subtree of that node and points to the right of the hyperplane are represented by the right subtree. The hyperplane direction is chosen in the following way: every node in the tree is associated with one of the k dimensions, with the hyperplane perpendicular to that dimension's axis. 
Both insertion takes $O(\log n)$. Worst case search is $O(n)$, but on average it is  $O(\log n)$.



\subsection{Radius Nearest Neighbours}

\paragraph{SNN}
Significantly improves over brute force and tree-based methods in terms of index and query time, provably returns exact results, and requires no parameter tuning. SNN exploits a sorting of the data points by their first principal component to prune the query search space. Further speedup is gained from an efficient implementation using high-level Basic Linear Algebra Subprograms (BLAS). See Figure~\ref{fig:SNN}

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/Screenshot 2025-01-02 at 09.21.36.png}
    \caption{Screenshot from \cite{chen2024fast}}
    \label{fig:enter-label}
\end{figure}


\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/Screenshot 2025-01-02 at 09.24.06.png}
    \caption{Screenshot from \cite{chen2024fast}}
    \label{fig:enter-label}
\end{figure}



\paragraph{GPU Powered Search}
A line of work translate fixed-radius nearest neighbour queries to ray tracing queries. Thus exploiting recent advances in GPU Hardware. The translation relies on a key observation: to find neighbours within a radius r of point p, we can expand a sphere of radius r around all points and check how many spheres contain the point p. The centres of the k-closest spheres are the neighbouring points of p.
Two recent works are by Nagarajan et.al.~\cite{nagarajan2023rt} for the Euclidian distance and Mandarapu et.al.~\cite{mandarapu2024arkade} for the general case. 
The latter compares against the following baselines:
SCANN which is a quantization-based approximate similarity search li-
brary; Treelogy which implements an exact KD-tree-based on a GPU;
FAISS which is a state-of-the-art exact quantization-based GPU library




\subsection{Approximate Methods}
Modern approaches generally focus on two aspects: indexing and sketching.
The indexing aims to construct a data structure that prunes the search space for a given query, hopefully resulting in fewer distance computations. Sketching, on the other hand, aims at reducing the cost of each distance computation by using a compressed approximate representation of the data \cite{chen2024fast}.


\paragraph{Tree Techniques}
The tree-based methods are known to become inefficient for high-dimensional data.
Tree based methods partition the state space using a tree structure. 
The overhead and construction time of the tree structures can be quite large but in exchange they offer fairly short query times.
Tree based methods can be used in conjunction with sketching to improve the performance. Trading exact results for probabilistic guarantees. 
For example, RP trees project data onto randomly chosen directions (hyperplanes) and split it into two halves based on the projection values.

\paragraph{Cell Techniques}
On the other hand, cell techniques create a regular grid, or hypercube, in the multidimensional domain and through a simple operation every point is assigned an integer lattice that points to its corresponding cell. A hash table can then be used for future queries, where the same operation is applied to the query point to know which cell it belongs to. The distance to every point in the cell, and probably in the contiguous cells as well, has to be computed to return only the points that meet the query condition. GriSPy is an implementation of such a technique \cite{chalela2021grispy}. They are closely related with Local Sensitivity Hashing.


\paragraph{Local Sensitivity Hashing}
Local Sensitivity Hashing (LHS) leverages a set of hash functions from the locality-sensitive hash family and it guarantees that similar queries are hashed into the same buckets with higher probability than less similar ones.

\subsection{Experimental Evaluations}

\paragraph{Syntetic Data}
Chen et.al.~\cite{chen2024fast} sample uniformly from $[0,1]^d$.


% \begin{table}[h!]
%     \centering
%     \small
%     \begin{tabular}{|c|p{4cm}|p{4cm}|p{4cm}|p{3cm}|}
%         \hline
%         \textbf{Sr No} & \textbf{Technique} & \textbf{Key Idea} & \textbf{Advantages} & \textbf{Disadvantages} & \textbf{Target Data} \\ \hline
%         1 & k Nearest Neighbor (kNN) [1] & Uses nearest neighbor rule & 
%         \begin{itemize}
%             \item Training is very fast
%             \item Simple and easy to learn
%             \item Robust to noisy training data
%             \item Effective if training data is large
%         \end{itemize} &
%         \begin{itemize}
%             \item Biased by value of \(k\)
%             \item Computation complexity
%             \item Memory limitation
%             \item Runs slowly as a lazy algorithm
%             \item Easily fooled by irrelevant attributes
%         \end{itemize} & Large data samples \\ \hline
%         2 & Weighted k Nearest Neighbor (WkNN) [2] & Assign weights to neighbors as per distance calculated & 
%         \begin{itemize}
%             \item Overcomes equal weight limitation of kNN
%             \item Uses all training samples
%             \item Global algorithm
%         \end{itemize} &
%         \begin{itemize}
%             \item Increases computational complexity
%             \item Algorithm runs slow
%         \end{itemize} & Large sample data \\ \hline
%         3 & Condensed Nearest Neighbor (CNN) [3,4,5] & Eliminate datasets that show similarity and do not add extra information & 
%         \begin{itemize}
%             \item Reduces size of training data
%             \item Improves query time and memory
%             \item Reduces recognition rate
%         \end{itemize} &
%         \begin{itemize}
%             \item Order-dependent
%             \item Unlikely to pick boundary points
%             \item Computational complexity
%         \end{itemize} & Memory-constrained datasets \\ \hline
%         % Continue similarly for other rows...
%     \end{tabular}
%     \caption{Comparison of Nearest Neighbor Techniques}
%     \label{tab:nn_comparison}
% \end{table}
